Quasi-polynomial-time algorithm for Independent Set in $P_t$-free graphs via shrinking the space of induced paths

In a recent breakthrough work, Gartland and Lokshtanov [FOCS 2020] showed a quasi-polynomial-time algorithm for Maximum Weight Independent Set in $P_t$-free graphs, that is, graphs excluding a fixed path as an induced subgraph. Their algorithm runs in time $n^{\mathcal{O}(\log^3 n)}$, where $t$ is assumed to be a constant. Inspired by their ideas, we present an arguably simpler algorithm with an improved running time bound of $n^{\mathcal{O}(\log^2 n)}$. Our main insight is that a connected $P_t$-free graph always contains a vertex $w$ whose neighborhood intersects, for a constant fraction of pairs $\{u,v\} \in \binom{V(G)}{2}$, a constant fraction of induced $u-v$ paths. Since a $P_t$-free graph contains $\mathcal{O}(n^{t-1})$ induced paths in total, branching on such a vertex and recursing independently on the connected components leads to a quasi-polynomial running time bound. We also show that the same approach can be used to obtain quasi-polynomial-time algorithms for related problems, including Maximum Weight Induced Matching and 3-Coloring.

==> prelim.tex <==
If not clearly stated otherwise, all logarithms are of base 2.
By $\comp(G)$ we denote the set of connected components of $G$.
For a graph $G$, we say that a set $X \subseteq V(G)$ is \emph{connected} if the graph $G[X]$ is connected.

%\begin{theorem}[Gy\'arf\'as~\cite{gyarfas}]\label{lem:ptfree-separator}
%Let $G$ be a $P_t$-free graph.
%Then there is a set $X$ of size at most $t$, such that every connected component of $G - N[X]$ has at most $|V(G)|/2$ vertices.
%Furthermore, such a set can be found in polynomial time.
%\end{theorem}

The following theorem is a crucial building block of our algorithms.
It was first observed by Gy\'arf\'as~\cite{gyarfas} for $P_t$-free graphs,
and then generalized by Chudnovsky \emph{et al.}~\cite{CPPT} for $C_{\geq t}$-free graphs.

\begin{theorem}[Gy\'arf\'as~\cite{gyarfas}, Chudnovsky \emph{et al.}~\cite{CPPT}]\label{lem:separator}
Let $G$ be a $C_{\geq t}$-free graph.
Then there is a connected set $X$ of size at most $t$, such that every connected component of $G - N[X]$ has at most $|V(G)|/2$ vertices.
Furthermore, such a set can be found in polynomial time.
\end{theorem}
